Towards Decentralized Heterogeneous Multi-Robot SLAM and Target Tracking

In many robotics problems, there is a significant gain in collaborative information sharing between multiple robots, for exploration, search and rescue, tracking multiple targets, or mapping large environments. One of the key implicit assumptions when solving cooperative multi-robot problems is that all robots use the same (homogeneous) underlying algorithm. However, in practice, we want to allow collaboration between robots possessing different capabilities and that therefore must rely on heterogeneous algorithms. We present a system architecture and the supporting theory, to enable collaboration in a decentralized network of robots, where each robot relies on different estimation algorithms. To develop our approach, we focus on multi-robot simultaneous localization and mapping (SLAM) with multi-target tracking. Our theoretical framework builds on our idea of exploiting the conditional independence structure inherent to many robotics applications to separate between each robot's local inference (estimation) tasks and fuse only relevant parts of their non-equal, but overlapping probability density function (pdfs). We present a new decentralized graph-based approach to the multi-robot SLAM and tracking problem. We leverage factor graphs to split between different parts of the problem for efficient data sharing between robots in the network while enabling robots to use different local sparse landmark/dense/metric-semantic SLAM algorithms.

==> Figures/approachGraph.tex <==
\begin{figure}[tb]
    
\begin{tikzpicture}[new set=import nodes]
 \begin{scope}[nodes={set=import nodes}]
     % Tracking Module
     % \node (x3t)[latent] at (2.5,1) {$x_3$};
     % SLAM Module a
      \node (x1)[latent] at (-1,-0.5) {$x_1^i$};
      \node [factor, right=of x1] (f1) {};
      \node [latent, right=of f1, xshift=-0.55cm] (x2) {$x_2^i$};
      \node [factor, right=of x2] (f2) {};
      \node [latent, right=of f2, xshift=-0.55cm] (x3) {$x_3^i$};
     
     \node [latent, above=of x3] (T3) {$T_3^i$};
     \node [factor, fill=red!100, between=x3 and T3] (ft3) {};
     \node [factor,  left=of T3] (f03) {};
     % \node [factor, fill=blue!100, below=of x3, yshift=0.2cm] (fs3) {};
     % \node [const, left=of fs3]  (title1) {\tiny Position from SLAM};

      
      % \node [factor, right=of x3] (f3) {};
      % \node [latent, right=of f3, xshift=-0.55cm] (x4) {$x_4$};
      
     
     % Map nodes
     \node [latent, below=of x3,xshift=-0.5cm] (l1) {$M^i$};
     \node [factor,  between=x1 and l1] (fl1) {};
     \node [factor, between=x2 and l1] (fl2) {};
     \node [factor,  between=x3 and l1] (fl3) {};
     % \node [factor, fill=blue!100, between=x4 and l1, label=right:\textcolor{blue!100}] (fl4) {};

         
    
     
  \end{scope}
  
 \graph {
    (import nodes);
     ft3--T3, f03--T3, ft3--x3,
    x1--f1, f1--x2, x2--f2, f2--x3,
    {x1,l1}--fl1, {x2,l1}--fl2,{x3,l1}--fl3,
    % fs3--[arrow, dashed]x3,

    
   };
    
\end{tikzpicture}

\end{figure}




==> Figures/approachGraph_b.tex <==
\begin{figure}[tb]
\centering
  
\begin{tikzpicture}[new set=import nodes]
 \begin{scope}[nodes={set=import nodes}]
     % robot i
      \node (x1)[latent] at (0,0) {$x_1^i$};
      \node [factor, below=of x1] (f1) {};
      \node [latent, below=of f1, yshift=0.55cm] (x2) {$x_2^i$};
      \node [factor, below=of x2] (f2) {};
      \node [latent, below=of f2, yshift=0.55cm] (x3) {$x_3^i$};
     
     \node [latent, right=of x3] (T3) {$T_{C,3}^{ij}$};
     \node [factor,  between=x3 and T3] (ft3) {};

     \node [latent, right=of x2, yshift=-0.55cm] (T3inj) {$T_{3}^{i\setminus j}$};
     \node [factor,  between=x3 and T3inj] (ft3inj) {};
     % \node [factor,  above=of T3] (f03) {};    
     
     % Map nodes
     \node [latent, left=of x2,yshift=-0.5cm] (l1) {$M^i$};
     \node [factor,  between=x1 and l1] (fl1) {};
     \node [factor, between=x2 and l1] (fl2) {};
     \node [factor,  between=x3 and l1] (fl3) {};

     % robot j
     \node [latent, right=of T3] (x3j) {$x_3^j$};
     \node [factor,  between=x3j and T3] (ft3j) {};
     \node [factor, above=of x3j] (f2j) {};
     \node [latent, above=of f2j, yshift=-0.55cm] (x2j) {$x_2^j$};
     \node [factor, above=of x2j] (f1j) {};
     \node [latent, above=of f1j, yshift=-0.55cm] (x1j) {$x_1^j$};

    
     % \node [latent, left=of x3j] (T3j) {$T_{C,3}^{ij}$};
     % \node [factor,  above=of T3] (f03j) {};    
     
     % Map nodes
     \node [latent, right=of x2j,yshift=-0.5cm] (l1j) {$M^j$};
     \node [factor,  between=x1j and l1j] (fl1j) {};
     \node [factor, between=x2j and l1j] (fl2j) {};
     \node [factor,  between=x3j and l1j] (fl3j) {};

     \begin{pgfonlayer}{background}
	% First rectangle
	\draw[fill=blue!10,rounded corners] (-2.25,-4.15) rectangle (0.5,0.5)
        node[above, xshift=-1.35cm] {SLAM $i$};
        \draw[fill=red!10,rounded corners] (3.15,-4.15) rectangle (5.9,0.5)node[above, xshift=-1.35cm] {SLAM $j$};
        \draw[fill=green!10,rounded corners] (0.75,-4.15) rectangle (2.9,-1.75)
        node[above, xshift=-1.05cm] {Tracking};
	
     \end{pgfonlayer}
     

         
    
     
  \end{scope}
  
 \graph {
    (import nodes);
     ft3--T3,  ft3--x3, %f03--T3,
    x1--f1, f1--x2, x2--f2, f2--x3,
    {x1,l1}--fl1, {x2,l1}--fl2,{x3,l1}--fl3,
    ft3inj--{x3,T3inj},
    
    ft3j--T3, ft3j--x3j,
    x1j--f1j, f1j--x2j, x2j--f2j, f2j--x3j,
    {x1j,l1j}--fl1j, {x2j,l1j}--fl2j,{x3j,l1j}--fl3j,
    % fs3--[arrow, dashed]x3,

    
   };
    
\end{tikzpicture}
    \caption{Factor graph representation of a 2-robot SLAM and target tracking application. Both robots $i$ and $j$ are building local maps $M^i$ and $M^j$ while cooperatively tracking targets in common $T^{ij}_C$ (observed at time step 3). The data  fused regarding common targets will indirectly update the map and the estimate of non-mutual targets $T^{i\setminus j}$.  }
      \label{fig:approachGraph}

\end{figure}




==> Figures/archit_1.tex <==
\begin{figure}[tb]
\centering
    
\begin{tikzpicture}[new set=import nodes]
 \begin{scope}[nodes={set=import nodes}]
     % Tracking Module
     \node (x3t)[latent] at (2.5,1) {$x_3^i$};
     
     \node [latent, above=of x3t] (T3) {$T_3^i$};
     \node [factor, fill=red!100, between=x3t and T3] (ft3) {};
     \node [latent, left=of x3t, yshift=1cm, xshift=-0.5cm] (x3cf) {$x_3^i$};
     % \node [factor,  left=of T3] (f03) {};
     \node [factor, fill=blue!100, left=of x3t] (fs3) {};
     \node [factor, fill=blue!100, below=of x3cf, yshift=0.15cm] (fs3cf) {};
     % \node [const, left=of fs3]  (title1) {\tiny Position from SLAM};

     

      % SLAM Module a
      \node (x1)[latent] at (-1,-0.5) {$x_1^i$};
      \node [factor, right=of x1] (f1) {};
      \node [latent, right=of f1, xshift=-0.55cm] (x2) {$x_2^i$};
      \node [factor, right=of x2] (f2) {};
      \node [latent, right=of f2, xshift=-0.55cm] (x3) {$x_3^i$};
      % \node [factor, right=of x3] (f3) {};
      % \node [latent, right=of f3, xshift=-0.55cm] (x4) {$x_4$};
      
     
     % Map nodes
     \node [latent, below=of x3,xshift=-0.5cm] (l1) {$M^i$};
     \node [factor,  between=x1 and l1] (fl1) {};
     \node [factor, between=x2 and l1] (fl2) {};
     \node [factor,  between=x3 and l1] (fl3) {};
     % \node [factor, fill=blue!100, between=x4 and l1, label=right:\textcolor{blue!100}] (fl4) {};

     \begin{pgfonlayer}{background}
	% First rectangle
	\draw[fill=blue!10,rounded corners] (-1.5,-2.75) rectangle (3,0)
        node[below, xshift=-3cm, yshift=-2.25cm] {SLAM Module};
        \draw[fill=green!10,rounded corners] (-1.5,3.25) rectangle (3,0.5)      node[above, xshift=-3cm, yshift=2.2cm] {Tracking Module};
        
        \draw[fill=red!10,rounded corners] (1.0,2.5) rectangle (-1,1) node[above, xshift=0.35cm, yshift=1cm] {CF};
	
     \end{pgfonlayer}

    
     
  \end{scope}
  
 \graph {
    (import nodes);
    x3t--ft3, ft3--T3, %f03--T3, %x3t--fs3,
    x1--f1, f1--x2, x2--f2, f2--x3,
    {x1,l1}--fl1, {x2,l1}--fl2,{x3,l1}--fl3,
    x3t--fs3, x3cf--fs3cf,
    fs3<-[dashed]x3, fs3cf<-[dashed]x3,
    % x3cf<->[dashed]x3t, x3cf<->[dashed]x3,

   };
    
\end{tikzpicture}
\caption{}
\label{fig:archit_1}



\end{figure}


==> Figures/chatGPTexample.tex <==
% \begin{figure}[tb]

% % Existing graph
% \begin{tikzpicture}[scale=2]
%   \draw[->] (-1,0) -- (1,0);
%   \draw[->] (0,-1) -- (0,1);
%   \draw[domain=-1:1,smooth,variable=\x,blue] plot ({\x},{\x*\x});
%   % \filldraw[fill=red!20, draw=red!50!black] ([shift={(1mm,-1mm)}]current page.north west) rectangle +(2cm,-2cm);
% \end{tikzpicture}

% % Rectangles
% \begin{tikzpicture}[remember picture, overlay]
%   % Background rectangle 1
%   \filldraw[fill=red!20, draw=red!50!black] ([shift={(1mm,-1mm)}]current page.north west) rectangle +(2cm,-2cm);
  
%   % Background rectangle 2
%   \filldraw[fill=green!20, draw=green!50!black] ([shift={(5mm,-5mm)}]current page.north west) rectangle +(3cm,-3cm);
  
%   % Background rectangle 3
%   \filldraw[fill=blue!20, draw=blue!50!black] ([shift={(10mm,-10mm)}]current page.north west) rectangle +(4cm,-4cm);
% \end{tikzpicture}

% \end{figure}


\begin{figure}[tb]

% \usetikzlibrary{backgrounds}

	
	\begin{tikzpicture}
		% Draw your graph here
		% \draw (0,0) -- (1,1) -- (2,0) -- cycle;
		
		% Draw the rectangle backgrounds
		\begin{pgfonlayer}{background}
			% First rectangle
			\draw[fill=blue!20,rounded corners] (-0.5,-0.5) rectangle (2,1);
			% Second rectangle
			\draw[fill=green!20,rounded corners] (2,-0.5) rectangle (4.5,1);
			% Third rectangle
			% \draw[fill=yellow!20,rounded corners] (-1.5,-1.5) rectangle (3.5,2.5);
		\end{pgfonlayer}
	\end{tikzpicture}


\end{figure}
